Spacetimes categories and disjointness for algebraic quantum field theory

An algebraic quantum field theory (AQFT) may be expressed as a functor from a category of spacetimes to a category of algebras of observables. However, a generic category $\mathsf{C}$ whose objects admit interpretation as spacetimes is not necessarily viable as the domain of an AQFT functor; often, additional constraints on the morphisms of $\mathsf{C}$ must be imposed. We introduce disjointness relations, a generalisation of the orthogonality relations of Benini, Schenkel and Woike (arXiv:1709.08657). In any category $\mathsf{C}$ equipped with a disjointness relation, we identify a subcategory $\mathsf{D}_\mathsf{C}$ which is suitable as the domain of an AQFT. We verify that when $\mathsf{C}$ is the category of all globally hyperbolic spacetimes of dimension $d+1$ and all local isometries, equipped with the disjointness relation of spacelike separation, the specified subcategory $\mathsf{D}_\mathsf{C}$ is the commonly-used domain $\mathsf{Loc}_{d+1}$ of relativistic AQFTs. By identifying appropriate chiral disjointness relations, we construct a category $\chi\mathsf{Loc}$ suitable as domain for chiral conformal field theories (CFTs) in two dimensions. We compare this to an established AQFT formulation of chiral CFTs, and show that any chiral CFT expressed in the established formulation induces one defined on $\chi\mathsf{Loc}$.

==> __preamble.tex <==
\usepackage[utf8]{inputenc}
\usepackage[UKenglish]{babel}
\usepackage[iso,UKenglish]{isodate}
\usepackage{csquotes}


\usepackage{enumitem} %for customizing labels in enumerate environments

%set textwidth to ~2.8 alphabets / 72-or-so characters per line
\newlength{\alphabet}
\settowidth{\alphabet}{\normalfont abcdefghijklmnopqrstuvwxyz}
\usepackage[a4paper,textwidth=2.8\alphabet]{geometry}


%prevent line breaks in inline math by increasing relevant penalties to maximum:
\relpenalty=10000
\binoppenalty=10000

%better typesetting stuff (should reduce overfull hboxes)
\usepackage{microtype}

%stuff for figures:
\usepackage[pdftex]{graphicx}
\usepackage{rotating}
\usepackage{subfig}

%stuff for prettier tables:
\usepackage{colortbl}


% stuff for mathematics:
\usepackage{mathtools}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{thmtools, thm-restate}
\usepackage{bbm} %for blackboard 1, use \mathbbm{1}
\usepackage{xfrac} %for nice split-level fractions, use \sfrac{numerator}{denominator}
\usepackage{faktor} %for typesetting quotient structures e.g. \faktor{X}{A}


% stuff for physics
\usepackage{slashed}
\usepackage{braket}
% \usepackage{feynmp-auto}
\usepackage{tensor}



% cross-referencing tools
% NB: package load order: amsmath, then hyperref, then cleveref.
\usepackage[colorlinks,linkcolor={blue},citecolor={red},urlcolor={blue}]{hyperref} % hyperlinks references; colorlinks option: use text colour rather than box to indicate hyperlink
% WARNING: text colour is printed, box is not. For print version, use:
% \hypersetup{hidelinks}
\usepackage[capitalise]{cleveref} % use \cref and \Cref commands for auto-formatted references
\crefname{equation}{}{}
\Crefname{equation}{Equation}{Equations}




% define own commands
\newcommand{\vc}[1]{\ensuremath{\mathbf{#1}}}
% \newcommand{\tr}{\ensuremath{\mathrm{tr}}}
\newcommand{\dd}{\ensuremath{\mathrm{d}}}
% \newcommand{\II}{\ensuremath{I\mkern-4mu I}}



% % create amsthm environments - separate counters for "postulates", "explanations", and theorem-types.
% \theoremstyle{definition}
% \newtheorem{definition}{Definition}%[chapter]
% \newtheorem{axiom}[definition]{Axiom}
% 
% \theoremstyle{remark}
% \newtheorem{example}{Example}[section]
% \newtheorem{remark}[example]{Remark}
% 
% \theoremstyle{plain}
% \newtheorem{proposition}{Proposition}%[chapter]
% \newtheorem{theorem}[proposition]{Theorem}
% \newtheorem{lemma}[proposition]{Lemma}
% \newtheorem{corollary}[proposition]{Corollary}
% \newtheorem{claim}[proposition]{Claim}




% create amsthm environments - same counter for "postulates" and theorem-types, and "explanations".
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\newtheorem{axiom}[definition]{Axiom}
\newtheorem{openquestion}[definition]{Open Question}

\theoremstyle{plain}
\newtheorem{proposition}[definition]{Proposition}
\newtheorem{theorem}[definition]{Theorem}
\newtheorem{lemma}[definition]{Lemma}
\newtheorem{corollary}[definition]{Corollary}
\newtheorem{claim}[definition]{Claim}

\theoremstyle{remark}
\newtheorem{example}[definition]{Example}
\newtheorem{remark}[definition]{Remark}















% % avoid widow+orphan lines
% \clubpenalty = 10000
% \widowpenalty = 10000
% \displaywidowpenalty = 10000



% % Format to add graphics:
%\begin{figure}[htbp]
%\centering
% %makebox command allows figure to be wider than text and remain centred.
%\makebox[\linewidth][c]{
%\subfloat[subcaption]{ \includegraphics[width/scaling]{filename}} \quad
%\subfloat[subcaption]{\includegraphics[width/scaling]{filename}}} \\
%\caption{caption}
%\label{fig:label}
%\end{figure}

